Using LLMs to Investigate Correlations of Conversational Follow-up Queries with User Satisfaction

With large language models (LLMs), conversational search engines shift how users retrieve information from the web by enabling natural conversations to express their search intents over multiple turns. Users' natural conversation embodies rich but implicit signals of users' search intents and evaluation of search results to understand user experience with the system. However, it is underexplored how and why users ask follow-up queries to continue conversations with conversational search engines and how the follow-up queries signal users' satisfaction. From qualitative analysis of 250 conversational turns from an in-lab user evaluation of Naver Cue:, a commercial conversational search engine, we propose a taxonomy of 18 users' follow-up query patterns from conversational search, comprising two major axes: (1) users' motivations behind continuing conversations (N = 7) and (2) actions of follow-up queries (N = 11). Compared to the existing literature on query reformulations, we uncovered a new set of motivations and actions behind follow-up queries, including asking for subjective opinions or providing natural language feedback on the engine's responses. To analyze conversational search logs with our taxonomy in a scalable and efficient manner, we built an LLM-powered classifier (73% accuracy). With our classifier, we analyzed 2,061 conversational tuples collected from real-world usage logs of Cue: and examined how the conversation patterns from our taxonomy correlates with satisfaction. Our initial findings suggest some signals of dissatisfactions, such as Clarifying Queries, Excluding Condition, and Substituting Condition with follow-up queries. We envision our approach could contribute to automated evaluation of conversation search experience by providing satisfaction signals and grounds for realistic user simulations.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> tables/axis1-by-satisfaction.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{The number of sessions having each Axis 1 theme between satisfactory sessions and unsatisfactory sessions. }
\label{tab:my-table}
\vspace{-0.25cm}

{\footnotesize\begin{tabularx}{\columnwidth}{@{}lXX@{}}
\toprule
                    & \textbf{Satisfactory sessions}                & \textbf{Unsatisfactory sessions} \\ \midrule
More                & Exploring Domain (37, 86.0\%)                 &  Narrowing Down (15, 100\%)           \\
Frequent            & Understanding Response (35, 81.4\%)           & Clarifying Queries (13, 86.7\%)       \\
                    & Clarifying Queries (31, 72.1\%)               & Understanding Response (9, 60.0\%)     \\
                    & Narrowing Down (29, 67.4\%)                   & Exploring Domain (7, 46.7\%)              \\
                    & Verifying Information (9, 20.9\%)             & Verifying Information (5, 33.3\%)        \\
                    & Seeking Different Representations (3, 6.98\%)         & Seeking Different Representations (3, 20.0\%)             \\
Less                & Unclassified (2, 4.65\%)                          & Reacting to Response (3, 20.0\%)         \\
Frequent            & Reacting to Response (0, 0\%)                 & Unclassified (1, 6.67\%)                        \\ \midrule
Total               & 43                                            & 15                                        \\ \bottomrule
\end{tabularx}}
\vspace{-0.25cm}

\end{table}

==> tables/axis1.tex <==
\begin{table*}[t]
\centering
\caption{Purpose of Follow-up Queries (Axis 1). Themes specific to conversational search are denoted with an asterisk (*). Relevant literature from the search domain is provided in the right column.}
\label{tab:axis1}

{\footnotesize\begin{tblr}{
  width=\textwidth,
  colspec={X[2.4]|X[2]|X[11]|X[1.3]},
  % cells={valign=m},
  row{1} = {c},
  cell{3}{1} = {r=2}{},
  cell{7}{1} = {r=2}{},
  vline{2-3} = {1-9}{},
  vline{3} = {-}{},
    vline{4} = {-}{},
  hline{1-2,3,5-7,9,10} = {-}{},
  hline{4,8} = {-}{Silver},
}
\textbf{Category}                          & \textbf{Theme}            & \textbf{Definition}                       & \textbf{Literature} \\
{\textbf{Clarifying Queries}}           &                               
& {When the user clarifies their search intent with the follow-up query.}                & {\cite{rha2017exploration, sahib2012comparative, jansen2007Patterns}} \\

{\textbf{Broadening\\Information}}       & Exploring Domain              
& {When users seek a broad understanding of a topic and ask questions in order to accomplish the same task.}        & {\cite{rha2017exploration}}\\
                                        & {Understanding \\Response}       
& {When the user finds the response lacking important information or hard to understand and tries to gather more information.}              & {\cite{athukorala2016exploratory}}\\
{\textbf{Deepening\\ Information}}        & Narrowing Down                
& {When the user seeks to obtain detailed and specific answers through the follow-up query.}  & {\cite{rha2017exploration}}    \\
{\textbf{Seeking Different\\ Representations}} & {}          
& {When the user seeks different representation (e.g. modality, format) to better understand the provided information } & {\cite{jansen2009Transition}}  \\
%                                 & {Organizing Information}          
% & {When the user desires to receive the information from the response in a specific format (e.g., list, table, visual materials, etc.).} & {\cite{jansen2009Transition}}  \\
{\textbf{Evaluating\\ Search Results}}    & {Verifying\\ Information}\mbox{*} 
& {When the user requests additional explanations, alternatives, or evidence regarding the accuracy, \\ completeness, or applicability of the information from the response.} & {-} \\
                                        & {Reacting to\\ Response}\mbox{*}  
& {When the user expresses the emotions of satisfaction or dissatisfaction or open ended feedback regarding the information provided by the response }  & {\cite{liao2020Conversational}} \\
\end{tblr}}


\end{table*}

% When the user explores the information from the response in a specific source (e.g., map, images, news, etc.).
% Exploring Different \\Types of Sources

==> tables/axis2-by-satisfaction.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{The number of sessions having each Axis 2 theme between satisfactory sessions and unsatisfactory sessions.}
\label{tab:axis2-by-satisfaction}
\vspace{-0.25cm}
{\footnotesize\begin{tabularx}{\columnwidth}{@{}>{\hsize=.25\hsize}XXX@{}}
\toprule
\textbf{                } & \textbf{Satisfactory sessions}                           & \textbf{Unsatisfactory sessions} \\ \midrule
{More\\Frequent}       & {Requesting Additional Information (37, 86.0\%)}          & {Requesting Additional Information (13, 86.7\%)} \\
                       & {Requesting Related Information (32, 74.4\%)}             & Adding/Specifying Condition (12, 80.0\%)  \\
                       & Adding/Specifying Condition (21, 48.8\%)                   & {Requesting Related Information (9, 60.0\%)}\\
                       & Substituting Condition (13, 30.2\%)                        & {Substituting Condition \& Excluding Condition \& Criticizing Response (each 5, 33.3\%)}  \\
                       & Confirming Response (10, 23.3\%)                           & Confirming Response (4, 26.7\%)\\
                       & Excluding Condition (7, 16.3\%)                            & Converting Format (3, 20.0\%)  \\
                       & Converting Format (3, 6.98\%)                              & Requesting Opinion (2, 13.3\%) \\
                       & {Criticizing Response \& Requesting Opinion (2, 4.65\%)} & Affirming Response (1, 6.67\%) \\
Less                   & Chatting Aimlessly (1, 2.33\%)                            &  Chatting Aimlessly  (0, 0\%)  \\
Frequent           & Affirming Response (0, 0\%)                                &  \\ \midrule
Total                                  & 43          & 15          \\ \bottomrule
\end{tabularx}}
\vspace{-0.25cm}

\end{table}

==> tables/axis2.tex <==


\begin{table*}[t]
\centering
\caption{Actions of follow-up queries (Axis 2). Themes specific to conversational search are denoted with an asterisk (*). Relevant literature from the search domain is provided in the right column.}
\label{tab:axis2}

{\footnotesize\begin{tblr}{
  width=\textwidth,
  colspec={X[1]|X[3]|X[9]|X[1]},
  % cells={valign=m},
  row{1} = {c},
  cell{2}{1} = {r=3}{c},
  cell{5}{1} = {r=5}{c},
  cell{10}{1} = {r=2}{c},
  cell{12}{1} = {c},
  % vline{1} = {-}{}
  vline{2-3} = {1-13}{},
  vline{4} = {1-13}{},
  vline{3} = {3-4,6-8,10-11}{},
  hline{1-2,5,10,12-13} = {-}{},
  hline{3-4,6-9,11} = {2-4}{Silver},
}
\textbf{Category}                          & \textbf{Theme}                & \textbf{Definition}                                                                       &\textbf{Literature}  \\
{\textbf{Query-}\\\textbf{specific}}    & Excluding Condition               & {When the user explicitly removes specific conditions from a previous query.}             & {\cite{rha2016Exploringa, rieh2006Analysis}}                                                     \\
                                        &{ Adding/Specifying Condition}       & {When the user specifies additional conditions or parameters to include in the query.}     & {\cite{trippas2018Informing, wang2009Broad, graesser2008question}}                                                    \\
                                        & Substituting Condition            & {When the user expresses the same query intent using different conditions or forms.}        & {\cite{rha2016Exploringa, rieh2006Analysis}}  \\
{\textbf{Response-}\\\textbf{specific}} & Converting Format\mbox{*}         & {When the user requests to receive the answer in a specific format (e.g., table, map, graph).}   & \cite{wang2009Broad}                                              \\
                                        & Criticizing Response\mbox{*}      & {When the user points out that the provided answer is unrelated or inappropriate to the original question.}  & {\cite{trippas2018Informing}} \\
                                        & Affirming Response\mbox{*}         & When the user expresses satisfaction with the provided answer.  & {\cite{trippas2018Informing}}  \\
                                        & {Requesting Additional Information} & When the user requests additional information related to the response.  & {\cite{trippas2018Informing}}  \\
                                        & Confirming Response                 & {When the user directly requests reconfirmation of the user's understanding or verifies previous response.} & {\cite{ashktorab2019resilient, cambazoglu2021intent}} \\
{\textbf{Session-}\\\textbf{specific}} & {Requesting Related Information}     & {When the user requests related information that is not directly referred in the response but related in the high-level domain}  & {\cite{boldi2011query}}                                                      \\
                                        & Requesting Opinion\mbox{*}          & {When the user asks additional information or opinion on the users’ own alternative options not previously referred in response.} & {-}                                 \\
\textbf{Misc.}                          & Chatting Casually\mbox{*}          & When the user attempts chitchat rather than seeking specific information. & {\cite{liao2020Conversational}} \\
                                        & Requesting Unrelated Information   & When the intent or content of the question is unclear.                    & {-} \\
\hline
\end{tblr}}
\end{table*}

